PokeFlex: A Real-World Dataset of Volumetric Deformable Objects for Robotics

Data-driven methods have shown great potential in solving challenging manipulation tasks; however, their application in the domain of deformable objects has been constrained, in part, by the lack of data. To address this lack, we propose PokeFlex, a dataset featuring real-world multimodal data that is paired and annotated. The modalities include 3D textured meshes, point clouds, RGB images, and depth maps. Such data can be leveraged for several downstream tasks, such as online 3D mesh reconstruction, and it can potentially enable underexplored applications such as the real-world deployment of traditional control methods based on mesh simulations. To deal with the challenges posed by real-world 3D mesh reconstruction, we leverage a professional volumetric capture system that allows complete 360{\deg} reconstruction. PokeFlex consists of 18 deformable objects with varying stiffness and shapes. Deformations are generated by dropping objects onto a flat surface or by poking the objects with a robot arm. Interaction wrenches and contact locations are also reported for the latter case. Using different data modalities, we demonstrated a use case for our dataset training models that, given the novelty of the multimodal nature of Pokeflex, constitute the state-of-the-art in multi-object online template-based mesh reconstruction from multimodal data, to the best of our knowledge. We refer the reader to our website ( https://pokeflex-dataset.github.io/ ) for further demos and examples.

==> tables/table-diff-cam.tex <==
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Input} &
  \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} &
  \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} &
  \textbf{$\text{RPFD} \downarrow$} &
  \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$} &
  \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$} \\ \midrule
Volucam   & \textbf{6.69}          & 8.38          & 0.698          & \textbf{7.433}          & 0.799          \\
RealSense & 7.91          & \textbf{7.37}          & \textbf{0.693}          & 7.675          & \textbf{0.806}          \\
Kinect    & 11.20         & 9.79         & 0.839         & 8.505         & 0.767          \\
Rendered  & 12.97         & 12.28        & 0.826         & 8.761         & 0.761 \ \\ 
Brighter RealSense   & 14.57         & 13.25        & 0.853         & 9.126         & 0.754 \ \\ 
Darker RealSense     & 13.89         & 11.74        & 0.957         & 9.831         & 0.736 \ \\ 
\bottomrule
\end{tabular}%
% \begin{tabular}{@{}lccccc@{}}
% \toprule
% \textbf{Input} &
%   \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} &
%   \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} &
%   \textbf{$\text{RPFD} \downarrow$} &
%   \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$} &
%   \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$} \\ \midrule
% Volucam   & 2.98          & 3.92          & 0.646          & 5.392          & 0.892          \\
% RealSense & 3.04          & 4.98          & 0.494          & 5.221          & 0.899          \\
% Kinect    & 4.21          & 6.32          & 0.752          & 6.456          & 0.845          \\
% Rendered  & \textbf{2.15} & \textbf{3.47} & \textbf{0.350} & \textbf{4.700} & \textbf{0.914} \\ \bottomrule
% \end{tabular}%
% }

% \footnotesize % or use \footnotesize for even smaller text
%     %\begin{adjustbox}{width=0.85\linewidth}
%         \begin{tabular}{lccccc} % Input % LPFD % LROI % J % RPFD
%         \textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} & \textbf{$\text{RPFD} \downarrow$} & \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}  \\ \hline
%         Volucam   
%         & 2.98          
%         & 3.92          
%         & 0.646 
%         & 5.392          
%         & 0.892          \\ \hline
%         RealSense 
%         & 3.04          
%         & 4.98  
%         & 0.494       
%         & 5.221         
%         & 0.899           \\ \hline
%         Kinect    
%         & 4.21          
%         & 6.32  
%         & 0.752        
%         & 6.456          
%         & 0.845          \\ \hline
%         Rendered  & \textbf{2.15} & \textbf{3.47} & \textbf{0.350}& \textbf{4.700} & \textbf{0.914}  \\ \hline
%     \end{tabular}
%     %\end{adjustbox}

==> tables/table-generalization-img-robot-data.tex <==

\begin{tabular}{p{2cm}cccc} % Input % LPFD % LROI % J % RPFD
\toprule
    \textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} 
% & \textbf{$\text{RPFD} \downarrow$} 
& \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}   \\ \midrule

\begin{tabular}[c]{@{}l@{}}Validation set \\(14 objects)\end{tabular}
& 5.13 $\pm$ 6.61          
& 4.26 $\pm$ 7.85
% & 0.648 $\pm$ 0.742
& 6.247 $\pm$ 2.731          
& 0.816 $\pm$ 0.105 \\ %\hline
Foam cylinder
& 4.77 $\pm$ 6.55          
& 2.42 $\pm$ 1.67
% & 0.629 $\pm$ 0.674
& 8.237 $\pm$ 3.928          
& 0.806 $\pm$ 0.093 \\ %\hline
Plush dice
& 2.94 $\pm$ 4.50          
& 3.59 $\pm$ 4.17
% & 0.571 $\pm$ 0.638
& 7.838 $\pm$ 1.905          
& 0.895 $\pm$ 0.036 \\ %\hline
Plush volleyball
& 2.48 $\pm$ 1.93          
& 3.52 $\pm$ 3.87
% & 0.175 $\pm$ 0.289
& 6.074 $\pm$ 1.510          
& 0.903 $\pm$ 0.034 \\ %\hline
Sponge
& 9.70 $\pm$ 9.13          
& 3.54 $\pm$ 2.31
% & 0.718 $\pm$ 0.764
& 8.673 $\pm$ 3.42          
& 0.711 $\pm$ 0.09 \\ %\hline
    \bottomrule
\end{tabular}


==> tables/table-generalization-pcd.tex <==

\begin{tabular}{p{2cm}ccccc} % Input % LPFD % LROI % J % RPFD
\toprule
\textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} 
% & \textbf{$\text{RPFD} \downarrow$} 
& \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}   \\ \midrule

\begin{tabular}[c]{@{}l@{}}Validation set \\(14 objects)\end{tabular}
& 5.13 $\pm$ 6.61          
& 4.26 $\pm$ 7.85
% & 0.648 $\pm$ 0.742
& 6.247 $\pm$ 2.731          
& 0.816 $\pm$ 0.105 \\ %\hline
Foam cylinder
& 4.77 $\pm$ 6.55          
& 2.42 $\pm$ 1.67
% & 0.629 $\pm$ 0.674
& 8.237 $\pm$ 3.928          
& 0.806 $\pm$ 0.093 \\ %\hline
Plush dice
& 2.94 $\pm$ 4.50          
& 3.59 $\pm$ 4.17
% & 0.571 $\pm$ 0.638
& 7.838 $\pm$ 1.905          
& 0.895 $\pm$ 0.036 \\ %\hline
Plush volleyball
& 2.48 $\pm$ 1.93          
& 3.52 $\pm$ 3.87
% & 0.175 $\pm$ 0.289
& 6.074 $\pm$ 1.510          
& 0.903 $\pm$ 0.034 \\ %\hline
Sponge
& 9.70 $\pm$ 9.13          
& 3.54 $\pm$ 2.31
% & 0.718 $\pm$ 0.764
& 8.673 $\pm$ 3.42          
& 0.711 $\pm$ 0.09 \\ %\hline
    \bottomrule
\end{tabular}


==> tables/table-objects-img-robot.tex <==
\begin{tabular}{p{3cm}cccccc} % Input % LPFD % LROI % J % RPFD
\toprule
\textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} & \textbf{$\text{RPFD} \downarrow$} & \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}   \\ \midrule
Beanbag
& 5.70          
& 7.59 
& 0.810
& 8.114          
& \textbf{0.825} \\ %\hline
Foam cylinder
& \textbf{2.10}          
& \textbf{1.43} 
& 0.623
& 6.807          
& \textbf{0.844} \\ %\hline
Foam dice
& \textbf{1.66}          
& 5.96
& 0.667
& \textbf{4.276}          
& \textbf{0.925}  \\ %\hline
Foam half sphere
& \textbf{0.80}          
& \textbf{1.12}            
& \textbf{0.272}        
& \textbf{2.622}          
& \textbf{0.928}\\ %\hline
Memory foam
& 22.27          
& 23.93            
& 1.585        
& 10.007          
& 0.588\\ %\hline
Pillow
& \textbf{0.84}          
& \textbf{0.96} 
& 0.625
& 9.092          
& \textbf{0.877}  \\ %\hline
Plush dice
& \textbf{2.47}          
& \textbf{2.35}
& 0.629
& 7.689          
& \textbf{0.902}  \\ %\hline
Plush moon
& \textbf{4.32}          
& \textbf{3.43}
& \textbf{0.518}
& \textbf{6.304}          
& \textbf{0.869}  \\ %\hline
Plush octopus
& \textbf{1.23}          
& \textbf{1.01}
& \textbf{0.536}
& \textbf{5.612}          
& \textbf{0.823}  \\ %\hline
Plush turtle
& \textbf{1.73}          
& \textbf{0.58} 
& 0.949
& 8.705          
& 0.760  \\ %\hline
Plush volleyball
& \textbf{2.45}          
& \textbf{2.57} 
& \textbf{0.166}
& \textbf{6.076}          
& \textbf{0.901}  \\ %\hline
Sponge
& \textbf{5.29}          
& \textbf{1.43} 
& \textbf{0.340}
& \textbf{6.439}          
& 0.791  \\ %\hline
Toilet paper roll
& 17.94          
& 22.80 
& \textbf{0.385}
& 7.651          
& 0.726  \\ %\hline
3D printed bunny
& 8.79          
& \textbf{3.86} 
& 0.791
& \textbf{6.284}          
& 0.722  \\ %\hline
3D printed cylinder
& \textbf{5.21}          
&  5.61
& 0.666
& \textbf{5.943}     
& \textbf{0.822}  \\ %\hline
3D printed heart
& 6.79          
& \textbf{4.17} 
& \textbf{0.294}
& \textbf{5.658}          
& 0.789  \\ %\hline
3D printed pyramid
& 5.43          
& \textbf{3.61}
& 0.878
& \textbf{5.617}          
& 0.705  \\ %\hline
    \bottomrule
\end{tabular}

==> tables/table-objects-img.tex <==
\begin{tabular}{p{3cm}cccccc} % Input % LPFD % LROI % J % RPFD
\toprule
\textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} & \textbf{$\text{RPFD} \downarrow$} & \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}   \\ \midrule
Beanbag
& \textbf{5.86}          
& 12.78 
& \textbf{0.467}
& 7.994          
& \textbf{0.833} \\ %\hline
Foam cylinder
& \textbf{5.87}          
& \textbf{7.61} 
& 1.366
& 9.300          
& 0.767 \\ %\hline
Foam dice
& \textbf{5.06}          
& 12.19
& 0.845
& \textbf{5.900}          
& \textbf{0.884}  \\ %\hline
Foam half sphere
& \textbf{0.81}          
& \textbf{2.24}            
& \textbf{0.229}        
& \textbf{2.640}          
& \textbf{0.927}\\ %\hline
Memory foam
& 9.34          
& 17.21            
& 0.978        
& \textbf{7.432}          
& 0.723\\ %\hline
Pillow
& \textbf{1.35}          
& \textbf{1.88} 
& 0.920
& 10.70          
& \textbf{0.840}  \\ %\hline
Plush dice
& \textbf{4.80}          
& \textbf{5.05}
& 0.823
& 9.511          
& \textbf{0.869}  \\ %\hline
Plush moon
& \textbf{3.85}          
& \textbf{6.73}
& \textbf{0.391}
& \textbf{5.437}          
& \textbf{0.890}  \\ %\hline
Plush octopus
& \textbf{2.28}          
& \textbf{2.09}
& 0.855
& \textbf{6.851}          
& 0.773  \\ %\hline
Plush turtle
& \textbf{2.10}          
& \textbf{0.89} 
& 1.174
& 9.268          
& 0.732  \\ %\hline
Plush volleyball
& 8.96          
& 15.73 
& \textbf{0.290}
& 9.083          
& \textbf{0.835}  \\ %\hline
Sponge
& 8.39          
& \textbf{4.71} 
& \textbf{0.513}
& 7.661          
& 0.734  \\ %\hline
Toilet paper roll
& 24.93          
& 37.33 
& \textbf{0.501}
& 9.055          
& 0.672  \\ %\hline
3D printed bunny
& 10.60          
& \textbf{4.38} 
& \textbf{0.677}
& \textbf{6.943}          
& 0.714  \\ %\hline
3D printed cylinder
& \textbf{5.04}          
&  \textbf{6.06}
& 0.777
& \textbf{6.005}     
& \textbf{0.820}  \\ %\hline
3D printed heart
& 8.17          
& \textbf{4.70} 
& \textbf{0.341}
& \textbf{6.115}          
& 0.764  \\ %\hline
3D printed pyramid
& \textbf{6.53}          
& \textbf{4.09}
& 0.988
& \textbf{5.725}          
& 0.695  \\ %\hline
    \bottomrule
\end{tabular}

==> tables/table-objects-pcd.tex <==
\begin{tabular}{p{3cm}cccccc} % Input % LPFD % LROI % J % RPFD
\toprule
\textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} & \textbf{$\text{RPFD} \downarrow$} & \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}   \\ \midrule
Beanbag
& 9.18          
& 8.63 
& 1.402
& 9.608          
& 0.790 \\ %\hline
Foam cylinder
& \textbf{0.73}          
& \textbf{0.67} 
& \textbf{0.337}
& \textbf{4.701}          
& \textbf{0.909} \\ %\hline
Foam dice
& \textbf{1.98}          
& \textbf{2.6}
& \textbf{0.414}
& \textbf{4.415}          
& \textbf{0.924}  \\ %\hline
Foam half sphere
& \textbf{0.32}          
& \textbf{1.41}            
& \textbf{0.148}        
& \textbf{2.202}          
& \textbf{0.952}\\ %\hline
Memory foam
& \textbf{4.54}          
& 8.26     
& \textbf{0.578}        
& \textbf{5.008}          
& 0.786\\ %\hline
Pillow
& \textbf{0.85}          
& \textbf{1.23} 
& 0.666
& 8.835          
& \textbf{0.882}  \\ %\hline
Plush dice
& \textbf{2.22}          
& \textbf{2.68}
& 0.583
& 7.433          
& \textbf{0.905}  \\ %\hline
Plush moon
& \textbf{0.68}          
& \textbf{1.15}
& \textbf{0.179}
& \textbf{3.546}          
& \textbf{0.946}  \\ %\hline
Plush octopus
& 4.88          
& \textbf{4.68}
& 1.310
& 8.937         
& 0.692  \\ %\hline
Plush turtle
& \textbf{1.22}          
& \textbf{0.89} 
& 0.98
& 8.076          
& 0.762  \\ %\hline
Plush volleyball
& \textbf{1.67}          
& \textbf{3.36} 
& \textbf{0.106}
& \textbf{5.307}          
& \textbf{0.921}  \\ %\hline
Sponge
& 5.28          
& \textbf{2.55} 
& \textbf{0.354}
& 7.237          
& 0.760  \\ %\hline
Toilet paper roll
& 14.13          
& 17.06 
& \textbf{0.314}
& 6.901          
& 0.742  \\ %\hline
3D printed bunny
& 12.22          
& 7.74 
& 0.883
& 7.289          
& 0.665  \\ %\hline
3D printed cylinder
& \textbf{3.06}          
&  \textbf{2.36}
& 0.573
& \textbf{4.834}     
& \textbf{0.858}  \\ %\hline
3D printed heart
& 9.91          
& 6.73 
& \textbf{0.488}
& 6.475          
& 0.754  \\ %\hline
3D printed pyramid
& \textbf{4.29}          
& 6.97
& 0.653
& \textbf{4.681}          
& 0.765  \\ %\hline
    \bottomrule
\end{tabular}

==> tables/table-performance.tex <==
%\begin{adjustbox}{width=\columnwidth}
        \begin{tabular}{p{2.5cm}ccccc} % Input % LPFD % LROI % J % RPFD
        \toprule
        \textbf{Input} & \textbf{$\mathcal{L}_{\text{PFD}} \cdot 10^3 \downarrow$} & \textbf{$\mathcal{L}_{\text{ROI}} \cdot 10^3 \downarrow$} 
        % & \textbf{$\text{RPFD} \downarrow$} 
        & \textbf{$\text{CD}_{\text{UL1}} \text{[mm]} \downarrow$}  & \textbf{$J(\mM_{\text{P}}, \mM_{\text{GT}}) \uparrow$}   \\ \midrule
        Images
        & 7.34 $\pm$ 13.45          
        & 7.22 $\pm$ 12.09 
        % & 0.708 $\pm$ 0.783
        & 7.547 $\pm$ 3.684         
        & 0.791 $\pm$ 0.126 \\ %\hline
        Robot data
        & 8.47 $\pm$ 13.57          
        & 5.50 $\pm$ 9.31
        % & 0.867 $\pm$ 0.934
        & 8.283 $\pm$ 3.719
        & 0.779 $\pm$ 0.111  \\ %\hline
        Images + robot data 
        & 6.64 $\pm$ 12.72          
        & 4.99 $\pm$ 10.58  
        % & 0.638 $\pm$ 0.716        
        & 7.025 $\pm$ 2.995          
        & 0.806 $\pm$ 0.110\\ %\hline
        
        \begin{tabular}[c]{@{}l@{}}Dense synthetic point \\ clouds (5k points)\end{tabular}
        & \textbf{4.34} $\pm$ 5.32
        & \textbf{3.64} $\pm$ 6.12
        % & 0.621 $\pm$ 0.832
        & \textbf{6.185} $\pm$ 2.409
        & \textbf{0.825} $\pm$ 0.105 \\
        \begin{tabular}[c]{@{}l@{}}Sparse synthetic point \\ clouds (100 points)\end{tabular} 
        & 4.84 $\pm$ 6.22 
        & 4.77 $\pm$ 7.52
        % & 0.611 $\pm$ 0.737
        & 6.445 $\pm$ 2.321
        & 0.823 $\pm$ 0.090 \\
        Kinect point clouds
        & 5.75 $\pm$ 10.54        
        & 5.00 $\pm$ 8.05   
        % & \textbf{0.597} $\pm$ 0.681   
        & 6.498 $\pm$ 2.59 
        & 0.820 $\pm$ 0.112 \\ %\hline
        \begin{tabular}[c]{@{}l@{}}Kinect point clouds \\+ robot data \end{tabular}
        & 5.68 $\pm$ 9.43      
        & 4.06 $\pm$ 6.86  
        % & 0.617 $\pm$ 0.728
        & 6.615 $\pm$ 2.871
        & 0.817 $\pm$ 0.115 \\ %\hline
% \begin{tabular}[c]{@{}l@{}}Sparse synthetic Point \\ Clouds (100 points)\end{tabular} & 3.72          & 5.30          & 0.640          & 5.513          & 0.851 \\ 
        \bottomrule
    \end{tabular}
    %\end{adjustbox}
